General Interpolation and Strong Amalgamation for Contiguous Arrays

Interpolation is an essential tool in software verification, where first-order theories are used to constrain datatypes manipulated by programs. In this paper, we introduce the datatype theory of contiguous arrays with maxdiff, where arrays are completely defined in their allocation memory and for which maxdiff returns the max index where they differ. This theory is strictly more expressive than the array theories previously studied. By showing via an algebraic analysis that its models strongly amalgamate, we prove that this theory admits quantifier-free interpolants and, notably, that interpolation transfers to theory combinations. Finally, we provide an algorithm that significantly improves the ones for related array theories: it relies on a polysize reduction to general interpolation in linear arithmetics, thus avoiding impractical full terms instantiations and unbounded loops.

==> eqint.tex <==

\subsection{Equality Interpolating and Beth Definability Properties}\label{subsec:equint}

In this section we give some more information about syntactic consequences of strong amalgamation (this information is partially new even with respect to~\cite{BGR14} and will be needed for designing an appropriate interpolation algorithm).

In~\cite{BGR14}[Proposition 5.7] the general interpolation property (and the strong amalgamation property equivalent to it) are shown to be equivalent to a Beth definability property for convex theories. We need a similar characterization for non convex theories in this paper, in order to improve  our interpolation algorithm from~\cite{ourfossacs}. 

First of all, we recall a third  characterization of strong amalgamation
in terms of the so-called \emph{equality interpolating property}. Equality interpolating property was introduced by Yorsh-Musuvathi in~\cite{yorsh} for convex theories and then extended to non-convec theories in~\cite{BGR14}.
% 
In fact,
there is a close relationship between the strong amalgamation
property of a theory $T$ and the fact that disjunctions of equalities
among variables are entailed, modulo $T$, by finite sets of atoms.
%
To make this precise, we need to introduce some preliminary notions.

Given two finite tuples $\ut\coincide t_1, \dots, t_n$ and
$\uv\coincide v_1,\dots, v_m$ of terms,
\begin{eqnarray*}
  \text{the notation }
  \ut \cap \uv \neq \emptyset 
   \text{ stands for the formula } 
  \bigvee_{i=1}^n \bigvee_{j=1}^m (t_i\uguale v_j) .
\end{eqnarray*} 
We use $\ut_1\ut_2$ to denote the juxtaposition of the two tuples
$\ut_1$ and $\ut_2$ of terms.  So, for example, $\ut_1\ut_2\cap \uv
\not= \emptyset$ is equivalent to $(\ut_1 \cap \uv \not= \emptyset)
\vee (\ut_2 \cap \uv \not= \emptyset)$.
\begin{definition}
  \label{def:eq-interpol}
  A theory $T$ is \emph{equality interpolating} iff it has the
  quantifier-free interpolation property and satisfies the following
  condition:
  \begin{itemize}
    \item
      for every quintuple $\ux, \uy_1,\uz_1, \uy_2, \uz_2$ of
      tuples of variables and for every pair of quantifier-free formulae
      $\delta_1(\ux, \uz_1,\uy_1)$ and $\delta_2(\ux,\uz_2, \uy_2)$
      such that
      \begin{equation}
        \label{eq:antecedent_var}
        \delta_1(\ux,\uz_1, \uy_1) \wedge 
        \delta_2(\ux,\uz_2, \uy_2) \vdash_T 
        \uy_1\cap \uy_2\neq \emptyset
      \end{equation}
      there exists a tuple $\uv(\ux)$ of terms such that
      \begin{equation}
        \label{eq:consequent_var}
        \delta_1(\ux, \uz_1,\uy_1)\wedge 
        \delta_2(\ux,\uz_2, \uy_2)\vdash_T 
        \uy_1\uy_2\cap \uv\neq \emptyset ~.
      \end{equation} 
  \end{itemize}
\end{definition}

Algorithms for computing the equality interpolating terms satisfying~\eqref{eq:consequent_var} are supplied for various convex theories in~\cite{yorsh}. For non-convex theories, in~\cite{BGR14} it is observed that such terms can be supplied by the `testing points' used for quantifier elimination in quantifier eliminating theories admitting a universal set of axioms~\cite{BGR14}[Theorem 4.4]. This is the case of theories of interests for the present paper (like `integer difference logic' \IDL, `unit-two-variable-per-inequality' \UTVPI, linear integer arithmetics, linear real arithmetics, etc.): however, a \emph{careful choice of the language} is needed to get such result, see again~\cite{BGR14} for details.

We now formally restate Theorem 4.2 from~\cite{BGR14}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}
  \label{thm:strong_amalgamation_syntactic}
  Given a universal theory $T$ having quan\-ti\-fier-free interpolation, 
  the following conditions are equivalent:
  \begin{description}
  \item[{\rm (i)}] $T$ is strongly amalgamable;
  \item[{\rm (ii)}] $T$ is equality interpolating.
 % \item[{\rm (iii)}] for every triple $\ux, \uy_1, \uy_2$ of tuples of
 %   variables and for every pair of quantifier-free formulae
 %   $\delta_1(\ux, \uy_1), \delta_2(\ux, \uy_2)$ such that
 %   \begin{equation}
 %     \label{eq:antecedent}
 %     \delta_1(\ux, \uy_1)\wedge \delta_2(\ux, \uy_2)\vdash_T
 %     \uy_1\cap \uy_2\neq \emptyset %\leqno\eqref{eq:antecedent}  
 %   \end{equation}
 %   there exists a tuple $\uv(\ux)$ of terms such that
 %   \begin{equation}
 %     \label{eq:consequent}
 %     \delta_1(\ux, \uy_1)\wedge \delta_2(\ux, \uy_2)\vdash_T
 %     \uy_1\uy_2\cap \uv\neq \emptyset ~.%\leqno\eqref{eq:consequent} 
 %   \end{equation}
  \end{description}
\end{theorem}

The convex formulation of the implicit and explicit definability properties for primitive formulae given in~\cite{ijcar20} can be extended to non-convex theories as follows. We keep the names `implicit/explicit definability' for simplicity, although it might be more appropriate to speak of
`implicit/explicit definability up to disjunctions' for the properties mentioned below.

\begin{definition}\label{def:expl}
 Let $T$ be a theory and let be $\delta(\ux,\uy)$ be a formula with free variables among $\ux, \uy$. We say that $\phi$ \emph{explicitly defines the $\uy$} (modulo $T$, using the $\ux$ as parameters) iff there is a tuple of terms $\ut(\ux)$ such that 
 \begin{equation}\label{eq:explicit}
  T\models \delta(\ux, \uy) \to \uy\cap \ut \neq \emptyset~~.
 \end{equation}
\end{definition}

\begin{definition}\label{def:impl}
 Let $T$ be a theory and let be $\delta(\ux,\uy)$ be a formula with free variables among $\ux, \uy$. We say that $\phi$ \emph{implicitly defines the $\uy$} (modulo $T$, using the $\ux$ as parameters) iff there is natural number $N>1$ such that 
 \begin{equation}\label{eq:implicit}
  T\models \bigwedge_{i=1}^N\delta(\ux, \uy^{(i)}) \to 
  \bigvee_{i=1}^N\bigvee_{j=i+1}^N (\uy^{(i)}\cap \uy^{(j)} \neq \emptyset)~~
 \end{equation}
 where the $\uy^{(i)}$ are renamed copies of the $\uy$.
\end{definition}

A formula is said to be \emph{existential} iff it is of the kind $\exists \uz\,\phi$ where $\phi$ is quantifier-free.
%a conjunction of literals.

\begin{theorem}\label{thm:beth}
 Let $T$ be a universal equality interpolating theory; then $T$ has the \emph{Beth definability property} for existential formulae, in the sense that for every existential formula $\delta(\ux, \uy)$, we have that $\delta$ implicitly defines the $\uy$ iff  it explicitly defines them. 
\end{theorem}

\begin{proof}
The proof is in the appendix.
 \end{proof}

In case the $SMT(T)$-problem is decidable,
explicit definability is semi-decidable by enumerating the tuples of terms $\ut$ required for~\eqref{eq:explicit} to hold. This is a highly impractical procedure; a better semi-decision procedures is suggested by Theorem~\ref{thm:beth}: one increases $N$ until the $T$-unsatisfiability test 
for the negation of~\ref{eq:implicit} is positive and at that point one can invoke the equality interpolating algorithm for $T$ to get the desired tuple $\ut$.

 

We underline that Definitions~\ref{def:expl},~\ref{def:impl} (and consequently also Theorem~\ref{thm:beth}) apply also to infinite sets of formulae $\Delta(\ux, \uy)$ containing at most the finitely many free variables $\ux, \uy$: simply sat that $\Delta$ explicitly (resp. implicitly) defines $\uy$ iff the conjunction $\bigwedge \Delta_0$ does, for a finite subset $\Delta_0\subseteq \Delta$.


==> metarules.tex <==

\subsection{Interpolating meta-rules}
\label{subsec:metarules}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\input{tablemr}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
The interpolation method for combination of theories relies on the
abstract framework---based on `meta-rules'---introduced
in~\cite{lmcs_interp} (to which, the interested reader is pointed
for more details) and used also in~\cite{BGR14}.  A meta-rule applies
(bottom-up) to a pair $A,B$ of finite sets of ground
formulae
producing an equisatisfiable pair of sets of formulae.  Each meta-rule
comes with a proviso for its applicability and an instruction for the
computation of the interpolant.  As an example, consider the meta-rule
(Define0):
\begin{center}
\small
\begin{tabular}{cll}
  $A\cup\{a=t\} \sep B\cup\{a=t\}$ 
  &~~
  \emph{Proviso}: $t$ is $AB$-common, $a$ is fresh \\ \cline{1-1}
  $A \sep B$ 
  & ~~
  \emph{Instruction}: $\phi' \coincide \phi(t/a)$.
\end{tabular}
\end{center}
%It is 
%not difficult to see 
%that 
$A\cup B$ is equisatisfiable to
$A\cup B\cup\{ a=t\}$ %since $a$ is a fresh variable that has been
%introduced to re-name the $AB$-common term $t$ %ale10jan2022: the explanation is trivial
according to the
\emph{proviso} of (Define0).  Its \emph{instruction} %of (Define0) %ale10jan2022
allows
for the computation of the interpolant $\phi'$ by eliminating the fresh
constant $a$ from the recursively %known  %ale10jan2022
constructed interpolant $\phi$.

The idea is to build an \emph{interpolating meta-rules refutation} for
a given unsatisfiable conjunction $A^0\wedge B^0$.  Such a refutation is a 
finite
labeled
tree having the following properties: (i) nodes are labeled by pairs
of finite sets of ground formulae; (ii) the root is labeled by $A^0,
B^0$; (iii) the leaves are labeled by a pair $\tilde A, \tilde B$ such
that $\bot \in \tilde A\cup \tilde B$; (iv) each non-leaf node is the
conclusion of a meta-rule
%%% from Table~\ref{tab:metarules} 
and its successors are the premises of that meta-rule (the complete
list of meta-rules is given in the appendix).  %ale10jan2022
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\input{tablemr}  %ale10jan2022
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Once an interpolating meta-rules refutation has been built, it is
possible to recursively compute the interpolant by using (top-down)
the instructions attached to the meta-rules in the tree as stated in
the following result.
\begin{proposition}[\hspace{.5pt}\cite{lmcs_interp}]
  \label{prop:metarules}
  If there exists an interpolating meta-rules refutation for $A^0, B^0$
  then there is a quan\-ti\-fier-free interpolant
 for $A^0, B^0$
  (i.e., there exists a quan\-ti\-fier-free \abcommon sentence $\phi$
  such that $A^0\vdash \phi$ and $B^0 \wedge \phi \vdash \bot$). The
  interpolant $\phi$ is recursively computed by applying the relevant
  interpolating instructions of %above the meta-rules. %ale2022
  the meta-rules above. %ale2022 non bisogna anche dire 'applying ... the instructions... top-down? mi sembra importante dirlo qui
\end{proposition}

%The idea to build the interpolation algorithm is the following.  
For our interpolation algorithm we %ale10jan2022
design transformation instructions to non-deterministically
apply to a pair $(A^0, B^0)$. Each of the transformation instructions
is \emph{justified by meta-rules}, in the sense that it is just a
special sequence of applications of meta-rules. Thus, metarules are not properly part of the algorithm, but %themselves; instead %ale10jan2022
 \emph{they constitute the proof that the algorithm is correct} (however, %they only guarantee partial correctness,  
termination is not guaranteed). %ale10jan2022 %achieved by metarules and requires a separate, non trivial argument).

The instructions are such that, whenever they are applied exhaustively
to a pair ($A^0, B^0$) such that $A^0\wedge B^0$ is unsatisfiable, they produce a
tree that is an interpolating meta-rules refutation for $A^0, B^0$
from which an interpolant can be extracted according to 
Proposition~\ref{prop:metarules}.

Before presenting our interpolation algorithm, we recall a technique, called \emph{Term Sharing},
from~\cite{lmcs_interp}.  Suppose that $A$ contains a literal $a
=t$, where the term $t$ is \abcommon and the free constant $a$ is
\astrict (a symmetric technique applies to $B$ instead of $A$). Then it
is possible to ``make $a$ \abcommon'' in the following way. First,
introduce a fresh \abcommon constant $c$ with the explicit definition
$c=t$ (to be inserted both in $A$ and in $B$, as justified by meta-rule
(Define0)); then replace the literal $a=t$ by $a=c$ and replace $a$ by
$c$ everywhere else in $A$; finally, delete $a=c$ too.  The result is
a pair $(A, B)$ where basically nothing has changed but $a$ has been
renamed to an \abcommon constant $c$ (the transformation can be easily
justified by %a suitable subset of the %ale10jan2022
meta-rules).


==> tablemr.tex <==

\vspace{5pt}
%Prime 4
\begin{multicols}{4}%\scriptsize
\textbf{Close1}
$$
\frac{}{A|B}
$$
Proviso: $A$ is unsatisfiable.

\noindent Instruction: $\phi'=\bot$.

\vspace{5pt}
\textbf{Close2}
$$
\frac{}{A|B}
$$
Proviso: $B$ is unsatisfiable.

\noindent Instruction: $\phi'=\top$.

\vspace{5pt}
\textbf{Propagate1}
$$
\frac{A|B\cup\{\psi\}}{A|B}
$$
Proviso: $A\vdash\psi$ and $\psi$ is $AB$-common.

\noindent Instruction: $\phi'=\phi\land \psi$.

\vspace{5pt}
\textbf{Propagate2}
$$
\frac{A\cup\{\psi\}|B}{A|B}
$$
Proviso: $B\vdash\psi$ and $\psi$ is $AB$-common.

\noindent Instruction: $\phi'=\psi\to \phi$.
\end{multicols}
\vspace{2pt}
%5-8
\begin{multicols}{4}%\scriptsize
\textbf{Define0}
$$
\frac{A\cup\{a=t\}|B\cup\{a=t\}}{A|B}
$$
Proviso: $t$ is $AB$-common, $a$ is new.

\noindent Instruction: $\phi'=\phi(t/a)$.

\vspace{5pt}
\textbf{Define1}
$$
\frac{A\cup\{a=t\}|B}{A|B}
$$
Proviso: t is $A$-local, $a$ is new.

\noindent Instruction: $\phi'=\phi$.

\vspace{5pt}
\textbf{Define2}
$$
\frac{A|B\cup\{a=t\}}{A|B}
$$
Proviso: $t$ is $B$-local, $a$ is new.

\noindent Instruction: $\phi'=\phi$.

\vspace{5pt}
\textbf{Disjunction1}
$$, 
\frac{...A\cup\{\psi_k\}|B...}{A|B}
$$
Proviso: $\lor_{k=1}^n \psi_k$ is $A$-local, $A\vdash \lor_{k=1}^n \psi_k$.

\noindent Instruction: $\phi'=\lor \phi_k$.
\end{multicols}
\vspace{2pt}
%9-12
\begin{multicols}{4}%\scriptsize
\textbf{Disjunction2}
$$
\frac{...A|B\cup\{\psi_k\}...}{A|B}
$$
Proviso: $\lor_{k=1}^n \psi_k$ is $B$-local and $B\vdash \lor_{k=1}^n \psi_k$.

\noindent Instruction: $\phi'=\land \phi_k$.

\vspace{5pt}
\textbf{Redplus1}
$$
\frac{A\cup\{\psi\}|B}{A|B}
$$
Proviso: $A\vdash\psi$ and $\psi$ is $A$-local.

\noindent Instruction: $\phi'=\phi$.

\vspace{5pt}
\textbf{Redplus2}
$$
\frac{A|B\cup\{\psi\}}{A|B}
$$
Proviso: $B\vdash\psi$ and $\psi$ is $B$-local.

\noindent Instruction: $\phi'=\phi$.

\vspace{5pt}
\textbf{Redminus1}
$$
\frac{A|B}{A\cup\{\psi\}|B}
$$
Proviso: $A\vdash\psi$ and $\psi$ is $A$-local.

\noindent Instruction: $\phi'=\phi$.
\end{multicols}
\vspace{2pt}
%13-16
\begin{multicols}{4}%\scriptsize
\textbf{Redminus2}
$$
\frac{A|B}{A|B\cup\{\psi\}}
$$
Proviso: $B\vdash\psi$ and $\psi$ is $B$-local.

\noindent Instruction: $\phi'=\phi$.

\vspace{5pt}
\textbf{ConstElim1}
$$
\frac{A|B}{A\cup\{a=t\}|B}
$$
Proviso: $a$ is $A$-strict and does not occur in $A,t$.

\noindent Instruction: $\phi'=\phi$.

\vspace{5pt}
\textbf{ConstElim2}
$$
\frac{A|B}{A|B\cup\{b=t\}}
$$
Proviso: $b$ is $B$-strict and does not occur in $B,t$.

\noindent Instruction: $\phi'=\phi$.

\vspace{5pt}
\textbf{ConstElim0}
$$
\frac{A|B}{A\cup\{c=t\}|B\cup\{c=t\}}
$$
Proviso: $c,t$ are $AB$-common e $c$ does not occur in $A,B,t$.

\noindent Instruction: $\phi'=\phi$.
\end{multicols}

\vspace{5pt}

